StableGarment: Garment-Centric Generation via Stable Diffusion

In this paper, we introduce StableGarment, a unified framework to tackle garment-centric(GC) generation tasks, including GC text-to-image, controllable GC text-to-image, stylized GC text-to-image, and robust virtual try-on. The main challenge lies in retaining the intricate textures of the garment while maintaining the flexibility of pre-trained Stable Diffusion. Our solution involves the development of a garment encoder, a trainable copy of the denoising UNet equipped with additive self-attention (ASA) layers. These ASA layers are specifically devised to transfer detailed garment textures, also facilitating the integration of stylized base models for the creation of stylized images. Furthermore, the incorporation of a dedicated try-on ControlNet enables StableGarment to execute virtual try-on tasks with precision. We also build a novel data engine that produces high-quality synthesized data to preserve the model's ability to follow prompts. Extensive experiments demonstrate that our approach delivers state-of-the-art (SOTA) results among existing virtual try-on methods and exhibits high flexibility with broad potential applications in various garment-centric image generation.

==> chapters/1-introduction.tex <==
\section{Introduction}
\label{sec:intro}
% P1
%Advancements in image synthesis have led to significant interest in the generation of photorealistic images that incorporate specific attributes such as garments on varied poses and backgrounds. This research domain, critical for applications ranging from e-commerce to virtual try-ons, demands a nuanced understanding of garment representation, pose alignment, and natural control of text descriptions within generated imagery. The capability to dynamically render garments across a spectrum of model poses and styles not only pushes the boundaries of digital fashion but also enhances the fidelity and versatility of virtual try-on technologies.
%Recent strides in image synthesis have catalyzed the generation of photorealistic images, integrating complex attributes like garment variations across diverse poses and backgrounds. This arena is pivotal for applications extending from e-commerce platforms to virtual try-on systems, necessitating a sophisticated grasp of garment representation, pose alignment, and the seamless incorporation of textual descriptors. The dynamic rendering of garments, adaptable to a wide range of poses and styles, not only advances the frontiers of digital fashion but significantly augments the fidelity and adaptability of virtual fitting solutions.
Recent advancements in image generation, especially with the advent of text-to-image diffusion models trained on extensive datasets, have revolutionized this field. A prime example is Stable Diffusion, an open-source model cited as \cite{ldm}, which allows a broad user base to easily generate images from textual prompts. The advancements in image generation impact almost all of the application domains, including a task with a large market cap, garment-centric generation.

%P2
%Traditional approaches in this space, predominantly centered around virtual try-on systems, leverage deep learning models to map garments onto target figures, accounting for pose, fabric dynamics, and user body dimensions. The recent advancements in diffusion models have led to big progress towards realistic garment fitting on standardized poses. The recovery of details and the naturalness of the synthesized images are far better than previous GAN-based methods. 
%Predominantly, virtual try-on methodologies have harnessed deep learning frameworks to accurately transpose garments onto target models, accounting for pose, fabric dynamics, and anatomical dimensions. The recent evolution of diffusion models has marked a notable leap forward, achieving unprecedented realism in garment adaptation to standardized poses, surpassing previous Generative Adversarial Network (GAN)-based approaches in detail recovery and image naturalness.
Garment-centric generation aims to generate images with a given garment, controlled by descriptions, target pose, or target user's image. A closely related task is virtual tryon\cite{zhu2023tryondiffusion,anydoor,dci-vton,dresscode,gp-vton,stableviton,}, and it's target is to put given garments onto given users' body. The recent evolution of diffusion models has marked a notable leap forward, achieving unprecedented realism in garment adaptation to standardized poses, surpassing previous Generative Adversarial Network (GAN)-based approaches in detail recovery and image naturalness.

%P3
%Despite these advancements, existing methodologies exhibit limitations when extended beyond conventional virtual try-on tasks. Let's analyze the requirements of both suppliers and customers first. For the suppliers, it is always a question of how to try different conceptual posters with the lowest budget. For the customers, it is intriguing to put on garments on their own body, while keeping their surroundings unchanged. Most of the previous works on virtual tryon focused on putting garments on the user's body with a clean background. Street Tryon proposed Shop2Street and Street2Street tasks to fullfile customers' need, as it supports virtual tryon in complex poses and complex backgrounds. For the suppliers' needs, they hope to know the best way to demonstrate their garments. It is always a question "how can we adjust the model and background easily and naturally?". Therefore, now it's a practice that putting garments on mannequin and inpainting the background and the model. 
% tryon不错，但是不够。从商家的角度看，需要快速尝试garment在不同模特、不同姿态、不同背景下的视觉效果。从消费者角度看，需要visualize garments on themselves within casual backgrounds。street tryon提出了一套设计，可以解决消费者的需求，但是生产者角度下的尝试仍不足没有被很好的解决。近期应用stable diffusion的方案，仅仅应用到了sd的图像先验，但抛弃了sd自身的灵活性和创造性。
Nonetheless, when venturing beyond traditional virtual try-on applications, prevailing methods encounter significant constraints. Evaluating the demands from both suppliers, seeking cost-effective methods for creating diverse conceptual visuals, and consumers, desiring to visualize garments on themselves within casual backgrounds, reveals a gap in current capabilities. While initiatives like Street Tryon have made strides towards accommodating complex poses and backgrounds, and fulfilling consumer desires, the question of efficiently and naturally modifying models and backdrops for suppliers persists. Recent advancements leveraging stable diffusion models hint at the potential for garment-driven image generation, yet often fall short of fully harnessing text-driven flexibility and stylistic versatility inherent in stable diffusion. 

%P4
%我们认为，如果能将sd自身的灵活性和创造性很好的保持，那么对于商家、艺术家、消费者都是很有帮助的。可以超低成本的进行衣服相关的创作、尝试，赋能电商场景效率提升。
Therefore, if we could integrate the consistency of the target garment while keeping the flexibility of stable diffusion, the resulting system could benefit a broader range of users, including but not limited to suppliers, customers, and even artists. This way, the cost of garment-centric creativity could be vastly reduced, boosting the effectiveness of commercial practices. 
%But it still costs a lot, how can we boost the efficiency 10 more times? Recent works based on stable diffusion open a door to garment-driven generation. However, most of them fail to fully exploit the capability of stable diffusion that text prompt and flexible style adjustment. In this work, we design GarmentDiffusion, a unified framework based on Stable Diffusion. In the framework, the core part is a garment appearance encoder that extracts details of the given garment. It consists of an appearance encoder, and a reference posing encoder. The appearance encoder is connected with stable diffusion Unet via additive self-attention injection. Two extra controlnets provide target user pose and image content. The benefit of this design, the model learns implicit alignment via poses, makes it generalizable for in-the-wild garment reference, and flexible to deal with different tasks. The additive injection separates self-attention calculation between the unet and reference branch, make it possible to switch the base models. Moreover, we reform the training data with diverse text prompts, making the well-trained model controllable by text prompts.

%P5
To this end, we introduce StableGarment, a unified framework based on Stable Diffusion. This framework is carefully designed to fully unleash the potential of Stable Diffusion. At its core featuring a novel garment appearance encoder. This encoder, composed of an appearance and a reference posing encoder, is linked to the stable diffusion U-Net through an innovative additive self-attention mechanism. Additional control networks fine-tune user poses and image context, fostering a model adept at learning implicit pose alignments for versatile, real-world garment applications. This additive approach decouples self-attention processes, enabling switching base-model for creative tryon. Furthermore, our reforged training dataset is enriched with diverse text prompts, and empowers text control over the generated output.

to sumup, our contribution is three folded:
\begin{enumerate}
    \item we proposed a unified framework to deal with garment driven generation tasks, including garment-centric text2image, garment-centric controllable text2image, garment-centric stylized image generation, and virtual tryon with flexible inputs.
    \item we proposed pose guided appearance encoder, makes the appearance encoder generalizable to shop garment image and in-the-wild image. And specifically designed an additive self-attention injection layer, to make the base model switchable to stylized models. 
    \item we evaluate the performance of our model on different benchmarks, it achieves state-of-the-art performance on all of them. Showcasing the advantage of our method. 
\end{enumerate}


%They struggle with the integration of garments in response to free-form text inputs, adaptation to non-standard or highly dynamic poses, and the application on stylized or significantly varied body models. The granularity required for detailed texture mapping, pose-specific garment deformation, and context-aware synthesis remains a challenge, underscoring the need for a more flexible and generalizable framework.


%Further, techniques such as semantic segmentation and pose estimation are integral to these systems, allowing for detailed garment texture and shape adaptation. 




% %1. The subject or title of your paper.
% Garment Centric Generation via Stable Diffusion Prior
% Garment Driven Generation via Implicit Posing Alignment

% %2. The main research question or hypothesis you are addressing.
% We designed a unified framework to deal with garment driven generation. The proposed framework could fullfile four tasks: 
% text+garment to image, 
% text + model pose + garment to image, 
% model pose + image content + garment to image, 
% and switch base models to put garments on stylized characters. 

% %3. The significance or relevance of your research.
% The well-studied virtual tryon task is a subtask of our framework, and the others can not be straightly achieved via virtual tryon methods. The framework is closely related to text2image, subject driven image generation, and inpainting.

% %4. Any specific methodology or approach you are using.
% In the model, the core part is a garment appearance encoder that extracts details of the given garment. It consists of an appearance encoder, and a reference posing encoder. 
% The appearance encoder is connected with stable diffusion Unet via additive self attention layers. In contrast of reference only method, the additive layers make it possible to switch the base model. 
% Two extra controlnets provides target user pose and image content. On the benefit of this design, the model learns implicit alignment via poses, makes it generalizable for in-the-wild garment reference, and flexible to deal with different tasks. 

% %5. The intended contribution or findings of your research.
% to sumup, our contribution is three folded:
% - we proposed a unified framework to deal with garment driven generation.
% - we propsed pose guided appearence encoder, makes the appearence encoder generalizable to in-cloth image and in-the wild image. And specifically designed a additive self-attention layer, to make the base model switchable. 
% - we achieves state-of-the-art performance on all tasks, especially on virtual tryon. 



==> chapters/2-relatedwork.tex <==
\section{Related Work}

\noindent \textbf{Virtual Try-on.} 
There are two main categories for virtual try-on approaches: 3D-based approaches~\cite{aggarwal2022layered, halimi2022pattern, korosteleva2022neuraltailor, majithia2022robust} and image-based virtual try-on~\cite{viton-hd, hr-viton, stableviton, ladi-vton, bai2022single, fenocchi2022dual, han2018viton, issenhuth2020not, dresscode, wang2018toward}. 3D-based virtual try-on methods can usually generate more flexible and accurate results at different views but these methods greatly depend on the 3D parametric human models and suffer from high computational cost and the lack of large-scale 3D try-on dataset. By contrast, image-based virtual try-on methods are more promising since they are light-weighted and can generate reasonable results by training on large-scale try-on datasets.

Many existing image-based virtual try-on methods consist of two stages. The first stage is responsible for warping, transforming the reference image to match the pose of the target individual. In the second stage, the warped garment is blended with the image of the target person. The warped garment is obtained by a warping module such as Thin Plain Spine (TPS) method~\cite{duchon1977splines}. The limitation of the TPS method lies in its constrained degrees of freedom~\cite{viton-hd}, which may not effectively handle complex scenarios where different parts of the garment undergo varying deformations~\cite{dci-vton,chen2023size}. In addition to TPS, a series of flow-based methods~\cite{viton-hd,gp-vton,bai2022single,dci-vton} have been proposed for establishing correspondences between the reference garment and corresponding regions of the human body. However, both TPS and flow-based methods may exhibit noticeable confusion in correspondence when significant deformations occur due to the lack of structural information about the garment~\cite{chen2023size}. Moreover, the multi-stage nature of these methods adds complexity to the overall process. In order to disentangle the shape and appearance, many methods~\cite{hr-viton,viton-hd,li2021toward} also incorporate segmentation maps as additional conditions to compensate for information loss caused by occlusion of parts of the human torso due to masks. Nowadays many methods rely on additional parsers such as semantic maps, and dense pose as these conditions help preserve original information such pose and shape. However,  WUTON~\cite{issenhuth2020not} and PF-AFN~\cite{ge2021parser} observed that parsed-based methods may yield unsatisfactory images with prominent artifacts, largely attributed to inaccurate parsing results. Several parsed-free methods~\cite{issenhuth2020not,ge2021parser,lin2022rmgn,he2022style} have emerged to circumvent the artifacts stemming from inaccurate parsing results. Although these methods avoid inaccurate segmentation from parsers, occlusion remain a challenge for both parser-based and parser-free methods as discussed in OccluMix~\cite{yang2023occlumix}. Artifacts caused by occlusion can be hardly solved with warping modules which involved eliminating part of garment. 

\noindent \textbf{Stable Diffusion}
In recent years, text-to-image diffusion models \cite{dalle, dalle2,ldm, Imagen, IF, sdxl, raphael, ediffi, glide, zeng2023ipdreamer} has made remarkable progress, particularly with the advent of diffusion models. Among them, Stable Diffusion \cite{ldm} trained diffusion models on larger datasets, further advancing the development of diffusion models and becoming the mainstream for image generation large models. Plenty of plug-ins made the stable diffusion eco-system accessible to different tasks. For controllable image generation, \cite{controlnet} utilize a duplicate U-Net structure with trainable parameters while keeping the original U-Net parameters static, facilitating controllable generation with other modal information, and T2I-adapter \cite{t2i} employs a lightweight adapter for controlling layout and style using different modal images. For injecting new subjects, 


\noindent \textbf{Diffusion-based Try-on.}
Diffusion Probabilistic Models (DPMs) have shown promising generative capacities in the field of image synthesis and editing, including text-to-image systhesis~\cite{ssr-encoder}, image-to-image translation~\cite{pada}, and image inpainting~\cite{lugmayr2022repaint}. If we regard virtual try-on as a conditional inpainting task, many existing conditional inpainting diffusion models~\cite{anydoor,paint-by-example} can be directly applied to virtual try-on. Unfortunately,  these methods struggle to cope with complex and diverse object deformations, resulting in difficulties preserving details such as logos and text. The diffusion models~\cite{ladi-vton,zhu2023tryondiffusion,seyfioglu2023dreampaint,dci-vton} specially designed for virtual try-on have shown inspiring performance recently. DCI-VTON~\cite{dci-vton} harnesses the capabilities of the diffusion model, and the integration of the warping module contributes to the generation of virtual try-on outcomes with authenticity and quality. Inspired by textual inversion~\cite{gal2022image}, LaDI-VTON~\cite{ladi-vton} generate pseudo words representing garment to tackle the virtual try-on task. TryOnDiffusion~\cite{zhu2023tryondiffusion} build cascaded diffusion models combined with several conditions such as human pose and garment pose to generate high-resolution try-on images with various body poses and shapes. StableVITON~\cite{stableviton} leverages the prior knowledge embedded within the pre-trained diffusion model and learns the semantic correspondence between clothing and the corresponding regions of the human body, thereby enhancing the fine details of the garments. WarpDiffusion~\cite{li2023warpdiffusion} incorporate warping garments into diffusion models with local cross attention to generate detailed try-on images. The diffusion models can exploit not only knowledge from pretraining data but a variety of conditions to tackle the try-on tasks, which enable superior performance along with heavy dependence on parsers. 

==> chapters/4-method.tex <==
\section{Proposed Method}

\begin{figure*}[!h]
    \centering
\includegraphics[width=1.0\linewidth]{images/method_v1.jpg}
    \caption{Overall schematics of our method. }
    \label{overview}
\end{figure*}

In this part, we first discuss preliminaries about diffusion models in Section~\ref{sec:Preliminary}, and then introduce the design of our StableGarment in Section~\ref{sec:Architecture}, where we'll reveal the overall architecture, the design of garment encoder, and the design of tryon controlnet. Finally, the specifics of our dataset, training and inference process are detailed in Section~\ref{sec:Training}.

\subsection{Preliminary}
\label{sec:Preliminary}
\noindent\textbf{Diffusion Model (DM).}
DM~\cite{ddpm, score-based} belongs to the category of generative models that denoise from a Gaussian prior $\mathbf{x_T}$ to target data distribution $\mathbf{x_0}$ by means of an iterative denoising procedure. The common loss used in DM is:
\begin{equation}
    L_{simple}(\bm{\theta}) := \mathbb{E}_{\mathbf{x_0}, t, \bm{\epsilon}}\left[\left\|\bm{\epsilon}-\bm{\epsilon_\theta}\left(\mathbf{x_t}, t\right)\right\|_2^2\right],
\end{equation}
where $\mathbf{x_t}$ is an noisy image constructed by adding noise $\bm{\epsilon} \in \mathcal{N}(\mathbf{0},\mathbf{1})$  to the natural image $\mathbf{x_0}$ and the network $\bm{\epsilon_\theta(\cdot)}$ is trained to predict the added noise. At inference time, data samples can be generated from Gaussian noise $\bm{\epsilon} \in \mathcal{N}(\mathbf{0},\mathbf{1})$ using the predicted noise $\bm{\epsilon_\theta}(\mathbf{x_t}, t)$ at each timestep $t$ with samplers like DDPM~\cite{ddpm} or DDIM~\cite{ddim}.

\noindent\textbf{Latent Diffusion Model (LDM).}
LDM~\cite{ldm} is proposed to model image representations in autoencoder’s latent space. LDM significantly speeds up the sampling process and facilitates text-to-image generation by incorporating additional text conditions. The LDM loss is:
\begin{equation}
    L_{LDM}(\bm{\theta}) := \mathbb{E}_{\mathbf{x_0}, t, \bm{\epsilon}}\left[\left\|\bm{\epsilon}-\bm{\epsilon_\theta}\left(\mathbf{x_t}, t, \bm{\tau_{\theta}}(\mathbf{c})\right)\right\|_2^2\right],
\end{equation}
where $\mathbf{x_0}$ represents image latents and $\bm{\tau_\theta(\cdot)}$ refers to the BERT text encoder~\cite{bert} used to encodes text description $\mathbf{c_t}$.

\noindent\textbf{Stable Diffusion (SD).}
SD is a widely adopted text-to-image diffusion model based on LDM. Compared to LDM, SD is trained on a large LAION~\cite{laion5b} dataset and replaces BERT with the pre-trained CLIP~\cite{clip} text encoder.

\subsection{Network Architecture}
\label{sec:Architecture}

\subsubsection{Overview.} The overall architecture of StableGarment can be found in Fig.\ref{fig:overview}. Our model consists of three parts, a texture encoder, a dual controlnet, and a pretrained stable diffusion model. We fix the pretrained stable diffusion's parameter, including both VAE and unet. On top of the unet, we build a trainable copy of the unet to take garment as inputs. The texture encoder is enforced with a reference pose branch, which is used for implicit alignment between the in-cloth image and the target pose. There's also a dual controlnet that takes input from pose image and image content. Both the textual encoder and controlnets are connected with the unet via an additive manner, enabling flexible model switching. 

\subsubsection{Garment Encoder.} The texture encoder takes the garment as input. A core requirement is to extract the very details of the garment. Inspired by the recent works \cite{reference-only, ip-adapter, controlnet}, our encoder is designed as a trainable copy of unet. The encoder is connected with the denoising unet through \textbf{additive self-attention (ASA)} layers. The motivation of this design is to inject reference information through multiple scales to get the finest details from the reference image, meanwhile keeping its model-switching capacity.

The additive self-attention is specifically designed to enable the encoder to plug into any stylized base-models. 
%In contrast to the commonly used concatenation of the keys and values from both reference and denoising unet in self-attention layers, our design makes additive self attention injection. 
Though several previous works studied to use self-attention connecting denoising unet and reference unet, their connection is designed in a concatenation manner as reference-only controlnet suggested. However, we found that the concatenated self attention always yields obvious artifacts when switching base-models. As shown in the Supplimentary, the similarity distribution shifted by a large margin when switching models, although in each group the distribution seems to be normal. As inspired by this finding, we reform the connection in an additive manner. %, which is to concatenate the keys and values from both reference and denoising unet so that the denoising unet could query both self and reference. 

Formally, given a reference garment image $I_G$ and its corresponding posing reference $P_G$, the garment encoder $E_g$ generate multi-layered $\{(K_n, V_n)_{n=1}^N\}$, where $k$ denotes the self-attention layer of the unet structure. The $K$s and $V$s are queried by the $Q^u_n$, the query tensor of the $n$-th self attention layer of the denoising unet. The output value $\mathit{S^u}$ of that self attention layer is formulated as \ref{Equ:Add}.
\begin{equation}
%\{(K_n, V_n)_{n=1}^N\}=E_g(I_G, E_c(P_G))
\{(K_n, V_n)_{n=1}^N\}=E_g(I_G)
\end{equation}

\begin{equation}
\label{Equ:Add}
\mathit{S^u_n}
=\underbrace{\operatorname{Attntion}\left(\mathbf{Q^u_n}, \mathbf{K^u_n}, \mathbf{V^u_n}\right)}_{\textrm{self attention}} 
+\underbrace{\operatorname{Attntion}\left(\mathbf{Q^u_n}, \mathbf{K^g_n}, \mathbf{V^g_n}\right)}_{\textrm{reference attention}},
\end{equation}
where $\operatorname{Attention}(\mathbf{Q},\mathbf{K},\mathbf{V})$ is the attention operator that calculate attention via query $Q$, key $K$, and value $V$. 

%The encoder itself can be further enhanced by a reference posing branch. We hope our textual encoder takes input of both garments from both the shop image and the model image. To deal with cloth references on a reference model, the model is required to know how the cloth texture performs on the reference's body. Therefore, we add a reference posing branch on the encoder, and being jointly trained with the encoder itself. Note that for some cases the reference posing doesn't exists, like the data in viton HD. This branch is only optional.

\subsubsection{Tryon ControlNet.}
To empower the StableGarment model with pixel-aligned control signals, we design a controlnet for pose control and virual tryon applications. This controlnet is required to understand user's content input as well as pose. As image input and pose input are closely related to each other, we put the dual condition into a unified manner. For virtual tryon, the input should be masked image $I_m$, inpainting mask $M$ and pose guidance $P$. While for pose gaidance generation without a image condition, we simply fill the masked image $I_m$ with zeros and inpainting mask $M$ with ones, indicating the whole image is required to be generated. 

The controlnet features are directly added to the pre-trained U-Net as the corresponding feature residual. Formally, the controlnet $E_c$ takes input of the three conditions, and the feature residuals are added to the denoising unet as Equ. \ref{Equ:Contorlnet}

\begin{equation}
\label{Equ:Contorlnet}
\mathit{R^u}=E_c(I_m \odot M \odot P)
\end{equation}
where $R^u$ represents feature residual of controlnet, and $\odot$ denotes the concatenation operation. 

\subsubsection{Text Prompt}
To retain the model's prompt-following capacity, we send different prompts to the reference unet and the denoising unet. The reference unet takes the category description of the garment as prompt, and the denoising unet takes the description of the target image as prompt. This way, the reference unet is easier to understand the correct dynamic of the input garment, and the denoising unet is still capable of generating images with flexible text prompts.

\subsection{Training Strategy and Inference}
\label{sec:Training}
\noindent\textbf{Dataset Preparation.}
We utilize pre-trained models to generate high-quality synthesized garment data, ensuring the precise and controllable garment-centric learning process, as can be found in Fig.\ref{Fig:data}. We divide our data engine into three modules:
\begin{itemize}
    \item \textbf{Parser.} The parser is designed to generate a parse map and dense map from an input image, comprising a pre-trained parsing segmentation network and uses Detectron2~\cite{detectron2}.
    \item \textbf{Tagger.} The tagger is designed to generate an accurate and complete text description given a target garment image. It employs CogVLM-chat~\cite{cogvlm} to generate text label and GPT4 to generate inpainting templates for the drawer module.
    \item \textbf{Drawer.} The drawer serves as the synthesized data generator by utilizing controlNet~\cite{controlnet} and pre-trained inpainting epiCRealism~\cite{epicinapint} model. 
\end{itemize}

\noindent\textbf{Learning Objectives.}
We employ a two-stage training strategy for our StableGarment. In the first stage, we only utilized vanilla data for the Garmnet try-on task and train our garment encoder to capture the clothing details while holding text editability. The loss objective in this stage is formulated as:
\begin{equation}
    L = \mathbb{E}_{z_0, t, I_{g}, p,\epsilon\in\mathcal{N}(0,1)} \left[ ||\epsilon - \epsilon_{\theta}||_2^2\right],
\end{equation}
where $p$ is the Densepose of target try-on image and $I_{g}$ is the garment reference input.
In the second stage, we frozen our garment encoder and further train our tryon controlnet, a variant controlnet which take densepose, cloth-agnostic image and cloth warp mask. We adopt the same learning objective as which used in the former stage.

\noindent\textbf{Inference.}
We employ inpainting pipeline to achieve both virtual try-on consistency and cloth-agnostic region preservation. Concretely, each updating step can be rewritten as:
\begin{equation}
    \epsilon_{t-1} = m \odot \epsilon_t + (1-m) \odot z_t^{tar},
\end{equation}
In this way, the background information and model detail can be successfully preserved. Also,  our method can apply more advanced inpainting technique, e.g. Repaint~\cite{repaint}.

For other tasks, we employ text2image pipeline, combined with different setups as shown in Tab.\ref{tab:tasks}
\begin{table}[]
    \centering
    \caption{The StableGarment is capable of performing various tasks. The configurations for performing different tasks are listed in the table.}
    \begin{tabular}{c|c|c|c|c}
         \toprule
         Task & Pipeline & Garment encoder & Base model & Controlnet  \\
        \midrule
         t2i& text2image & $\checkmark$ & stable diffusion v1.5 & $\times$ \\
         stylized t2i & text2image & $\checkmark$ & stylized base-model & $\times$ \\
         controllable t2i & text2image & $\checkmark$ & any base-model & any contorlnets \\
         virtual tryon & inpainting & $\checkmark$ & stable diffusion v1.5 & tryon controlnet \\
         \bottomrule
    \end{tabular}
    \label{tab:tasks}
\end{table}


==> chapters/5-experiment_bak.tex <==
\section{Experiments}

\noindent\textbf{Baselines.} 
For subject-driven generation, we compare our method with three finetuning-free method, including ELITE~\cite{elite}, IP-Adapter~\cite{ip-adapter} and BLIP-Diffusion~\cite{blipdiffusion}. 
In the context of virtual try-on task, we compare our method with three GAN-based virtual try-on methods, VITON-HD~\cite{viton-hd}, HR-VITON~\cite{hr-viton} and GP-VTON~\cite{gp-vton}, and three Diffusion-based virtual try-on methods, LADI-VTON~\cite{ladi-vton}, DCI-VTON~\cite{dci-vton} and StableVITON~\cite{stableviton}. We also compare our method with diffusion-based inpainting methods, Paint-by-Example~\cite{paint-by-example} and AnyDoor~\cite{anydoor}. To ensure a fair comparison, we utilize the official implementations for all the aforementioned methods.

\noindent\textbf{Datasets.} 
For subject-driven generation, we introduce a garment-centric generation benchmark derived from a subset of the VITON-HD test set. This benchmark, which includes 14 garments and 6 text prompts, aims to cover a broad spectrum of garment attributes such as color, shape, pattern, size, and type. The prompts, crafted through GPT-4, integrate a diverse range of skin tones, hairstyles, backgrounds, and additional attributes, enabling a robust evaluation against subject-driven generation approaches.

In the context of the virtual try-on task, we employ two widely-used, publicly available high-resolution datasets for virtual try-on: VITON-HD~\cite{viton-hd} and Dress Code~\cite{dresscode}.
We keep the same train-test split as the previous methods~\cite{stableviton, ladi-vton} on both of these datasets. In our study, we only use the official datasets for training the virtual try-on tasks to ensure fairness.
% VITON-HD contains 13,679 frontal-view woman and top clothes image pairs at the resolution of 1024×768. Following previous work\cite{viton-hd, stableviton}, we split the dataset into a training set and a test set with 11,647 and 2,032 pairs, respectively, and conduct experiments at two different resolution. DressCode dataset features over 53,000 image pairs of clothing and human models wearing them. The dataset includes high-resolution images (i.e., 1024×768) and garments belonging to different macro-categories, such as upper-body clothes, lower-body clothes, and dresses. In our experiments, we focus on the upper clothes and employ the original splits of the dataset following previous methods~\cite{stableviton, ladi-vton}.

%We also build a garment-centric genearation benchmark. To compare with subject-driven methods, we make a benchmark composed of a subset of VITON-HD test set. The benchmark is consisted of 14 garments and 6 prompts. We selected the benchmark with consideration for covering a comprehensive range of garment categories, including factors such as color, shape, decorative patterns, size, and type. The prompts are generated by GPT-4, incorporating various skin colors, hair styles, backgrounds, and other attributes.


\begin{figure*}[!t]
    \centering
    \vspace{-0.0cm}
\includegraphics[width=1.0\linewidth]{images/t2i_v4.jpg}
    \caption{Comparison with subject-driven generation methods.}
    \label{t2i-comp}
        \vspace{-0.4cm}
\end{figure*}

\noindent\textbf{Evaluation Metrics.} %For fairness, we only use the official dataset to train virtual try-on task. Following previous methods, we employ SSIM~\cite{ssim} and LPIPS~\cite{lpips} for paired settings and FID~\cite{fid} and KID~\cite{kid} for unpaired settings. We incorporate human perception by conducting a user study for a more thorough comparison. 
For virtual try-on task, we keep consistent with previous methodologies and apply SSIM~\cite{ssim} and LPIPS~\cite{lpips} metrics for evaluation under paired settings, and FID~\cite{fid} and KID~\cite{kid} metrics for unpaired settings. Following previous studies~\cite{ssr-encoder,avrahami2023break,ruiz2023dreambooth,voynov2023p+}, we utilize the DINO-M metric to assess the fidelity of the generated image to the reference image. The DINO-M metric compares a masked version of the try-on image with the garment image and computes the similarity using image embeddings extracted by the DINO~\cite{caron2021emerging} model, reflecting the identity of the garment. As the objectives of subject-driven generation differ from try-on, we employ several distinct metrics CLIP-T, CLIP-I~\cite{hessel2021clipscore} and Aesthetic score~\cite{laion5b} to compare with subject-driven generation methods. 
%SSIM measures the quality of three key features: luminance, contrast, and structure between the reconstruction results and the ground truth.
%LPIPS evaluates the perceptual similarity. 
%FID and KID is computed for evaluating the generation performance. Following previous studies~\cite{ssr-encoder,avrahami2023break,ruiz2023dreambooth,voynov2023p+}, we utilize the Dino-M metric to assess the fidelity of generated image to the reference image. The Dino-M metric compares a masked version of the try-on image with the reference garment image, and computes the similarity using image embeddings extracted by the DINO model, reflecting the identity of the garment.
%We have gathered composite images created by various methods for 300 randomly chosen pairs from the test set, with a resolution of 512 × 384. We enlisted 20 human evaluators to identify which method best reconstructs the clothing and which yields the most lifelike outcomes for each pair. Subsequently, we tally and present the number of times each method is preferred as the top performer in these two categories.
%Implementation details will be provided in the supplementary material. 

To integrate human judgment into our evaluation process, we also conduct a comprehensive user study. In our experimental setup, we compiled composite
images generated by various methods for 100 randomly selected pairs from the test set. Totally 200 evaluators was tasked with determining which method most accurately reconstructs the clothing and which produces the most realistic outcomes for each pair. The results, showcasing the frequency with which each method was selected as the top choice in these categories and the average evaluation scores, based on their relative ranking order will be detailed and discussed. The user study and implementation details will be provided in the supplementary material. 



\subsection{Qualitative Results}

\begin{figure*}[!t]
    \centering
\includegraphics[width=1.0\linewidth]{images/vitonhd_v4.jpg}
    \caption{Qualitative comparison with baselines on VITON-HD dataset.}
    \label{viton-hd-comp}
    \vspace{-0.5cm}
    
\end{figure*}

\begin{figure*}[!t]
    \centering
\includegraphics[width=1.0\linewidth]{images/dresscode_v3.jpg}
    \caption{Comparison on Dress Code dataset.}
    \label{dresscode-comp}
        \vspace{-0.6cm}
\end{figure*}



\noindent \textbf{Subject-driven Generation Results.} 
Fig.~\ref{t2i-comp} displays our StableGarment can generate reasonable outputs following the different prompts while preserving clothing texture under different diffusion base models. BLIP-Diffusion and IP-Adapter can only preserve partial texture features of the garment, making them prone to losing details such as shape and text. In contrast, our method not only achieves better fidelity in texture, shape, and detail preservation but also offers adaptability in style transfer when switching base models.

\noindent \textbf{Virtual Try-on Results.} Fig.~\ref{viton-hd-comp} shows a visual comparison of our outputs to other baselines on VITON-HD. Although previous methods synthesize reasonable warping garments and preserve the background well, they tend to generate blurry try-on results with manifest artifacts. Diffusion-based methods greatly improve the garment generation quality, but most of these methods fail to capture accurate clothing texture, e.g. text and tiny patterns. Due to the meaningful feature spaces of our proposed garment encoder, the try-on cloth successfully preserves the slight details. For example, our method accurately captures the `ADIDAS' on the cloths in the last two rows. The quantitative results on VTION-HD convincingly verify that our method can achieve a more realistic try-on effect for these clothes. More examples of our virtual try-on results will be reported in the supplementary materials.
    
We also provide a visual comparison of our outputs to other baselines on Dress Code in Fig.~\ref{dresscode-comp}. Both GP-VTON and LADI-VTON tend to bring distinct artifacts and misinterpret details of clothing such as flower pattern and text, whereas our method better preserves these aspects. 

\subsection{Quantitative Results}

\noindent\textbf{Comparison with Subject-driven Generation Methods.} We propose a garment-centric benchmark as described above to evaluate our method and other baselines, which includes 14 garments and 6 different prompts. Table~\ref{Tab:subject} provides a detailed quantitative evaluation of these methods. Overall, both IP-Adapter and our method demonstrate the ability to generate accurate outputs that adhere to the given text descriptions. Moreover, our method clearly outperforms previous state-of-the-art fine-tuning-free methods on the CLIP-I and Aesthetic score metrics, showcasing the capability of our garment encoder to capture comprehensive and fine-grained features from reference garments.

\begin{table}[!t]
  \small       %此处写字体大小控制命令 
  \centering      %表格居中
  \setlength{\abovecaptionskip}{0cm}
  \caption{Quantitative comparison of subject-driven generation methods. Bold denote the best and underline denote the second best result.}         %表标题
  \vspace{-0.2cm}
  \label{Tab:subject}         %标签，用作引用
\begin{tabular}{l|ccc}
  \toprule
  \textbf{Model}                         & CLIP-T$\uparrow$    & CLIP-I$\uparrow$ & AS$\uparrow$ \\
  \midrule
  BLIP-Diffusion~\cite{blipdiffusion}     &  0.187            & \underline{0.692}     &    4.973         \\
  IP-Adapter~\cite{ip-adapter}            &  \textbf{0.274}            & 0.628        &    \underline{5.165}         \\
  ELITE~\cite{elite}                     &  0.244                & 0.617             &    4.468       \\
  Ours                                   &  \underline{0.262}              & \textbf{0.719}                  &   \textbf{5.255}         \\
  \bottomrule
\end{tabular}
\vspace{-0.2cm}
\end{table}

% \begin{table}[!t]
%   \small       %此处写字体大小控制命令 
%   \centering      %表格居中
%   \setlength{\abovecaptionskip}{0cm}
%   \caption{Quantitative comparison on VITON-HD dataset. We multiply KID by 100 for better comparison.}         %表标题
%   \label{Tab:main}
%   \vspace{-0.2cm}
% \scalebox{0.75}{%标签，用作引用
% \begin{tabular}{l|ccccc | ccccc}
%   \toprule
%    & \multicolumn{5}{c|}{\textbf{512x384}} & \multicolumn{5}{c}{\textbf{1024x768}} \\
%   \textbf{Model} & \textbf{LPIPS}↓  & \textbf{SSIM}↑ & \textbf{FID}↓ &\textbf{KID}↓ & \textbf{DINO-M}↑ & \textbf{LPIPS}↓  & \textbf{SSIM}↑ & \textbf{FID}↓ &\textbf{KID}↓ & \textbf{DINO-M}↑ \\
%   \midrule
%   VITON-HD~\cite{viton-hd}  &  0.117  & 0.862 & 12.12 & 0.323 & 0.615 
%                             &  0.126  & \underline{0.867} & 12.12 & \underline{0.318} & 0.615 \\
%   HR-VTON~\cite{hr-viton}   &  0.105  & 0.868 & 11.27 & 0.273 & 0.634 
%                             &  \underline{0.107}  & \textbf{0.880} & 12.24 & 0.375 & 0.634 \\
%   LADI-VTON~\cite{ladi-vton}&  0.092  & 0.875 & 9.37 & 0.158 & 0.633 
%                             &  -  & - & - & - & -\\
%   DCI-VTON$^*$~\cite{dci-vton}  &  0.092  & 0.876 & 9.44 & 0.164 & 0.648 
%                             &  -  & - & - & - & -\\
%   StableVITON~\cite{stableviton}   &  0.083  & 0.866 & \underline{8.19} & \underline{0.118} & 0.647 
%                             &  -  & - & - & - & - \\
%   GP-VTON$^*$~\cite{gp-vton}&  \underline{0.083}  & \textbf{0.887} & 9.83 & 0.141 & \textbf{0.675} 
%                             &  0.186  & 0.855 & 34.34 & 3.311 & \underline{0.645} \\
%   WarpDiffusion$^*$~\cite{}&  \underline{0.083}  & \textbf{0.887} & 9.83 & 0.141 & \textbf{0.675} 
%                             &  0.186  & 0.855 & 34.34 & 3.311 & \underline{0.645} \\
%   Paint-by-Example~\cite{paint-by-example}   &  0.217  & 0.776 & 14.17 & 0.825 & 0.590 
%                             &  0.262  & 0.760 & 23.69 & 1.482 & 0.485 \\
%   AnyDoor~\cite{anydoor}    &  0.139  & 0.828 & 12.73 & 0.544 & 0.641 
%                             &  0.173  & 0.804 & \underline{11.42} & 0.451 & 0.641 \\
%   Ours   &  \textbf{0.077}  & \underline{0.877} & \textbf{7.98} & \textbf{0.104} & \underline{0.661} 
%                             & \textbf{0.096} & 0.862 & \textbf{8.91} & \textbf{0.222} & \textbf{0.655} \\
%   \bottomrule
% \end{tabular}}
% \vspace{-0.2cm}
% \end{table}

\begin{table}[!t]
  \small       %此处写字体大小控制命令 
  \centering      %表格居中
  \setlength{\abovecaptionskip}{0cm}
  \caption{Quantitative comparison on VITON-HD dataset. We multiply KID by 100 for better comparison.}         %表标题
  \label{Tab:main}
  \vspace{-0.2cm}
\scalebox{0.95}{%标签，用作引用
\begin{tabular}{l|ccccc}
  \toprule
  \textbf{Model} & \textbf{LPIPS}↓  & \textbf{SSIM}↑ & \textbf{FID}↓ &\textbf{KID}↓ & \textbf{DINO-M}↑  \\
  \midrule
  VITON-HD~\cite{viton-hd}  &  0.117  & 0.862 & 12.12 & 0.323 & 0.615 \\
  HR-VTON~\cite{hr-viton}   &  0.105  & 0.868 & 11.27 & 0.273 & 0.634 \\
  LADI-VTON~\cite{ladi-vton}&  0.092  & 0.875 & 9.37 & 0.158 & 0.633 \\
  DCI-VTON$^*$~\cite{dci-vton}  &  0.092  & 0.876 & 9.44 & 0.164 & 0.648 \\ 
  StableVITON~\cite{stableviton}   &  0.083  & 0.866 & \underline{8.19} & \underline{0.118} & 0.647 \\
  GP-VTON$^*$~\cite{gp-vton}&  \underline{0.083}  & \textbf{0.887} & 9.83 & 0.141 & \textbf{0.675} \\
  Paint-by-Example~\cite{paint-by-example}   &  0.217  & 0.776 & 14.17 & 0.825 & 0.590 \\
  AnyDoor~\cite{anydoor}    &  0.139  & 0.828 & 12.73 & 0.544 & 0.641 \\
  Ours   &  \textbf{0.077}  & \underline{0.877} & \textbf{7.98} & \textbf{0.104} & \underline{0.661} \\
  \bottomrule
\end{tabular}}
\vspace{-0.2cm}
\end{table}



\noindent\textbf{Comparison with Visual Try-on Methods.} We compare our method with existing baselines on the VITON-HD dataset and report the results in Table~\ref{Tab:main}. Our method outperforms all the baselines in both 512$\times$384 and 1024$\times$768 resolution settings, particularly in the unpaired metrics (i.e., FID and KID).  The success of our approach can be attributed to the garment encoder and DensePose-based try-on ControlNet, which effectively capture fine-grained garment features and generate high-quality try-on images. Furthermore, we utilize DINO-M to evaluate the recovery of the cloth texture in the unpaired setting. Under this metric, our method displays competitive performance in both resolution settings, further demonstrating the superiority of our method in the virtual try-on task.






\begin{table}[!t]
  \small       %此处写字体大小控制命令 
  \centering      %表格居中
  \setlength{\abovecaptionskip}{0cm}
  \caption{User Study on virtual try-on task. We evaluate our methods with other four baselines on three metrics: Clothing texture, Try-on quality and Cloth-agnostic preservation.}         %表标题
  \label{Tab:userstudy}      
  \vspace{-0.2cm}
  \scalebox{0.85}{%标签，用作引用
\begin{tabular}{l|ccc | ccc}
  \toprule
  & \multicolumn{3}{c|}{\textbf{Human Preference(\%)\uparrow}} & \multicolumn{3}{c}{\textbf{Human Scores\uparrow}} \\
  \textbf{Model}                    & Texture          & Quality        & Preservation      & Texture       & Quality         & Preservation\\
  \midrule
  GP-VTON~\cite{gp-vton}            &  \underline{15.35}          & 13.82          &    15.85          & \underline{2.98}          & 2.72            & 2.68    \\
  DCI-VTON~\cite{dci-vton}          &  13.68           & 12.51          &    15.13          & 2.82          & 2.64            & 2.78    \\
  LADI-VTON~\cite{ladi-vton}        &  10.88           & 12.56          &    14.06          & 2.12          & 2.22            & 2.41      \\
  StableVITON~\cite{stableviton}    &  13.40           & \underline{14.32}          &    \underline{22.77}          & 2.69          & \underline{2.99}            & \textbf{3.02}   \\
  Ours                              &  \textbf{46.70}  & \textbf{46.80} &   \textbf{27.30}  & \textbf{3.15} & \textbf{3.12}   & \underline{2.99}    \\
  \bottomrule
\end{tabular}
\vspace{-0.4cm}
\end{table}

\subsection{User Study}
To further evaluate the generation quality of our model, we conduct a user study to measure both the realism of the generated images and their coherence with the inputs given to the virtual try-on model. Following previous work~\cite{stableviton}, we asked participants to identify images that performed best according to three criteria: texture, quality, and preservation. As shown in Table \ref{Tab:userstudy}, the results indicate that a higher percentage of participants favored the images generated by our method across all evaluation criteria. When measured by actual ratings, our methods get scores comparable to StableVITON in terms of preservation, but surpass other methods in all other aspects.

\subsection{Ablation Study}
We take the 512 $\times$ 384 resolution on the VITON-HD dataset as the basic setting and perform ablation studies to validate the effectiveness of each component of our method.

\noindent\textbf{Additive Self-Attention.} To study the effectiveness of our ASA operator, we built a model with concatenated self-attention and trained with the same setup. The qualitative and quantitative comparison can be found in Fig. \ref{Fig:ab-comp} and Table \ref{Tab:ASA} . When testing under standard setup, the quantitative performance of both models is compatible. However, when switching the base models into stylized ones, it is visually obvious that the images generated via the CSA model often suffer from unavoidable artifacts. Especially when the text prompt becomes complex, such as a detailed background description, the CSA model often misinterprets the attributes of the garment. Instead, the ASA counterpart generates stylized images with better quality. Both details of the garment and style of the base model can be well preserved by the ASA model.


\begin{table}[!t]
  \small       %此处写字体大小控制命令 
  \centering      %表格居中
  \setlength{\abovecaptionskip}{0cm}
  \caption{Ablation study for garment-centric generation. For User result “a / b”, a is
frequency that each method is chosen as the best result for restoring the clothes, and b represents the best generated result following the text description.}         %表标题
\vspace{-0.2cm}
  \label{Tab:ASA}         %标签，用作引用
	\resizebox{1\linewidth}{!}{% 
\begin{tabular}{l|ccc | ccc | ccc}
  \toprule
    & \multicolumn{3}{c|}{\textbf{SD1.5}} & \multicolumn{3}{c|}{\textbf{Anythingv5~\cite{anything}}} & \multicolumn{3}{c}{\textbf{Disney Pixar~\cite{disney}}} \\ 
    \textbf{Ablation Setups} & CLIP-T↑      & User(\%)↑  & AS↑ & CLIP-T↑      & User(\%)↑  & AS↑ & CLIP-T↑      & User(\%)↑  & AS↑\\
  \midrule
  Ours(w/o ASA)              &  0.328           & 32.57/38.24         & 5.430      
                             &  0.332           & 21.83/25.14         & 5.860       
                             &  0.316           & 10.78/22.30         & 5.631\\
  Ours(w/o Synthesized data) &  0.254           & 35.04/28.71         & 5.107       
                             &  0.275           & 12.29/14.86         & 5.625
                             &  0.280           & 24.71/12.99         & 6.02 \\
  Ours(full)                 &  0.327           & 32.38/33.04         & 5.598       
                             &  0.321           & 65.87/60.00         & 5.919
                             &  0.314           & 64.50/64.71         & 5.865\\
  \bottomrule
\end{tabular}}
\vspace{-0.2cm}
\end{table}

\noindent\textbf{Effects of Synthesized Data.} We also ablate the benefits of using synthesized data. The comparing setups are: 1) training with VITON-HD and 2) training with our synthesized data. Beyond standard viton benchmarks, we create a collection of diverse text prompt templates to generate images, and adopt \textbf{CLIP-T} to evaluate the prompt following capacity of each setup. From Table \ref{Tab:ASA}, we found that on the VITON-HD benchmark, their performances are close. However, when testing the prompt following capacity, the model trained with synthesized data significantly outperforms its counterpart. From Fig. \ref{Fig:ab-comp}, the images generated by the model trained without synthesized data would display monotonous backgrounds, which reflects a characteristic of the VITON-HD dataset. 

\begin{figure*}[!t]
    \centering
\includegraphics[width=1.0\linewidth]{images/ab_v4.jpg}
\vspace{-15pt}
    \caption{Effects of our proposed components. }
    \label{Fig:ab-comp}
\vspace{-0.6cm}
\end{figure*}

\begin{table}[!tb]
  \small       %此处写字体大小控制命令 
  \centering      %表格居中
  \setlength{\abovecaptionskip}{0cm}
  \caption{Ablation study for try-on ControlNet.}         %表标题
  \label{Tab:ab-quan-tab}         %标签，用作引用
  \vspace{-0.2cm}
\begin{tabular}{l|ccccc}
  \toprule
  Ablation Setups            & LPIPS↓   & SSIM↑   & FID↓  & KID↓  & DINO-M↑ \\
  \midrule
  Inpainting                 &  0.097       & 0.852         & 9.11     & 0.303         & 0.661        \\
  +OpenPose                  &  0.080       & 0.870         & 8.60     & 0.251         & 0.663        \\
  +DensePose(Ours)           &  0.077      & 0.877         & 8.02     & 0.110         & 0.661    \\
  \bottomrule
\end{tabular}
\vspace{-0.4cm}
\end{table}

\noindent\textbf{Comparison with Different Try-on ControlNet.} We evaluate three types of try-on ControlNet, with three different control inputs: (1) clothing-agnostic input and mask, (2) clothing-agnostic input, mask and OpenPose, and (3) clothing-agnostic input, mask, and DensePose. Fig.~\ref{Fig:ab-comp} shows a visual comparison of these three different setups of try-on ControlNets. All of these ControlNets enable to preserve detailed clothing texture due to our proposed garment encoder. However, without the aid of geometric information, it is difficult for our model to generate accurate human body, including arms and hands. In comparison to OpenPose control, DensePose control offers more geometric information. As shown in Fig.~\ref{Fig:ab-comp}, replacing OpenPose with DensePose as a condition results in the disappearance of artifacts caused by occulusion in the generated images, with the thickness of the arms also better matching real images. We also conduct a comprehensive quantitative experiment to verify the effectiveness of our proposed DensePose-based try-on controlnet. As presented in Table~\ref{Tab:ab-quan-tab}, when adding the OpenPose condition on top of the base inpainting ControlNet, all metrics improve, as the model gains more information about the human body structure. Replacing OpenPose with DensePose leads to improvements in the detailed morphology of the human body, and all metrics also show enhancements.
%\noindent \textbf{Reference Posing Branch}. 

% \subsubsection{Effectiveness of Finetuning} We also replace the finetuned controlnets with pretrained ones, to verify if the finetuning is necessary. 



% \noindent \textbf{}. 
